Deep Neural Network Fingerprinting by Conferrable Adversarial Examples

In Machine Learning as a Service, a provider trains a deep neural network and gives many users access. The hosted (source) model is susceptible to model stealing attacks, where an adversary derives a surrogate model from API access to the source model. For post hoc detection of such attacks, the provider needs a robust method to determine whether a suspect model is a surrogate of their model. We propose a fingerprinting method for deep neural network classifiers that extracts a set of inputs from the source model so that only surrogates agree with the source model on the classification of such inputs. These inputs are a subclass of transferable adversarial examples which we call conferrable adversarial examples that exclusively transfer with a target label from a source model to its surrogates. We propose a new method to generate these conferrable adversarial examples. We present an extensive study on the irremovability of our fingerprint against fine-tuning, weight pruning, retraining, retraining with different architectures, three model extraction attacks from related work, transfer learning, adversarial training, and two new adaptive attacks. Our fingerprint is robust against distillation, related model extraction attacks, and even transfer learning when the attacker has no access to the model provider's dataset. Our fingerprint is the first method that reaches a ROC AUC of 1.0 in verifying surrogates, compared to a ROC AUC of 0.63 by previous fingerprints.

==> tables/imagenet-model-acc.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Dataset}                                                                          & \textbf{Type}              & \textbf{Test Accuracy} & \textbf{\begin{tabular}[c]{@{}c@{}}Fingerprint \\ Accuracy\end{tabular}} & \textbf{Type} & \textbf{Test Accuracy} & \textbf{\begin{tabular}[c]{@{}c@{}}Fingerprint \\ Accuracy\end{tabular}} \\ \hline
\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}Image-\\ Net32\\ $\mathcal{D}_1$\end{tabular}} & \multicolumn{3}{c|}{\multirow{2}{*}{\textbf{Training Surrogate}}}                                                              & \multicolumn{3}{c|}{\multirow{2}{*}{\textbf{Training Reference}}}                                                 \\
                                                                                          & \multicolumn{3}{c|}{}                                                                                                          & \multicolumn{3}{c|}{}                                                                                             \\ \cline{2-7} 
                                                                                          & \textbf{ResNet20 (Source)} & 0.557                  & 1.00                                                                     & -             & -                      & -                                                                        \\ \cline{2-7} 
                                                                                          & ResNet20                   & {[}0.539, 0.555{]}     & 1.00                                                                     & ResNet20      & {[}0.539, 0.569{]}     & 0.00                                                                     \\ \cline{2-7} 
                                                                                          & ResNet56                   & {[}0.551,0.564{]}      & 1.00                                                                     & ResNet56      & {[}0.5612, 0.601{]}    & 0.00                                                                     \\ \cline{2-7} 
                                                                                          & Densenet                   & {[}0.533,0.535{]}      & 1.00                                                                     & Densenet      & {[}0.536, 0.560{]}     & 0.00                                                                     \\ \cline{2-7} 
                                                                                          & VGG19                      & {[}0.553, 0.566{]}     & 1.00                                                                     & VGG19         & {[}0.534, 0.541{]}     & 0.00                                                                     \\ \cline{2-7} 
                                                                                          & MobileNetV2                & {[}0.586, 0.591{]}     & 1.00                                                                     & MobileNetV2   & 0.638                  & 0.00                                                                     \\ \hline
\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}Image-\\ Net32\\ $\mathcal{D}_2$\end{tabular}} & \multicolumn{3}{c|}{\multirow{2}{*}{\textbf{Testing Surrogate}}}                                                               & \multicolumn{3}{c|}{\multirow{2}{*}{\textbf{Testing Reference}}}                                                  \\
                                                                                          & \multicolumn{3}{c|}{}                                                                                                          & \multicolumn{3}{c|}{}                                                                                             \\ \cline{2-7} 
                                                                                          & MobileNetV2                & {[}0.5264, 0.531{]}    & {[}0.96, 0.98{]}                                                         & MobileNetV2   & {[}0.627, 0.631{]}     & {[}0.58, 0.64{]}                                                         \\ \cline{2-7} 
                                                                                          & ResNet20                   & {[}0.531, 0.532{]}     & {[}0.96, 0.98{]}                                                         & ResNet20      & {[}0.543, 0.557{]}{]}  & {[}0.44, 0.50{]}                                                         \\ \cline{2-7} 
                                                                                          & ResNet56                   & {[}0.542, 0.549{]}     & {[}0.98, 1.00{]}                                                         & ResNet56      & {[}0.589, 0.593{]}     & 0.5                                                                      \\ \cline{2-7} 
                                                                                          & Densenet                   & {[}0.499, 0.520{]}     & {[}0.82, 0.98{]}                                                         & Densenet      & {[}0.556, 0.563{]}     & {[}0.38, 0.56{]}                                                         \\ \cline{2-7} 
                                                                                          & VGG19                      & {[}0.519, 0.531{]}     & 0.76                                                                     & VGG19         & {[}0.528, 0.554{]}     & {[}0.28, 0.40{]}                                                         \\ \hline
\end{tabular}

==> tables/imagenetremoval.tex <==
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Dataset}                                                                           & \textbf{Type}                 & \multicolumn{1}{l|}{\textbf{Attack $\mathcal{A}$}} & \textbf{\begin{tabular}[c]{@{}c@{}}Test\\ Acc\end{tabular}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}FP\\ Acc\end{tabular}}} \\ \hline
\multirow{28}{*}{\begin{tabular}[c]{@{}c@{}}Image-\\ net32\\ $\mathcal{D}_2$\end{tabular}} & \multicolumn{4}{c|}{\textbf{Model Extraction}}                                                                                                                                                                                    \\ \cline{2-5} 
                                                                                           & ResNet20                      & Jagielski                                          & 0.532                                                       & 0.98                                                                           \\ \cline{2-5} 
                                                                                           & ResNet20                      & Papernot                                           & 0.509                                                       & 0.90                                                                           \\ \cline{2-5} 
                                                                                           & ResNet20                      & Knockoff                                           & 0.474                                                       & 0.98                                                                           \\ \cline{2-5} 
                                                                                           & \multicolumn{4}{c|}{\textbf{Fine-Tuning}}                                                                                                                                                                                         \\ \cline{2-5} 
                                                                                           & ResNet20                      & FTLL                                               & 0.573                                                       & 1.00                                                                           \\ \cline{2-5} 
                                                                                           & ResNet20                      & FTAL                                               & 0.613                                                       & 1.00                                                                           \\ \cline{2-5} 
                                                                                           & ResNet20                      & RTLL                                               & 0.590                                                       & 1.00                                                                           \\ \cline{2-5} 
                                                                                           & ResNet20                      & RTAL                                               & 0.45                                                        & 0.82                                                                           \\ \cline{2-5} 
                                                                                           & \multicolumn{4}{c|}{\textbf{Adversarial Training}}                                                                                                                                                                                \\ \cline{2-5} 
                                                                                           & ResNet20                      & FGM                                                & 0.554                                                       & 1.00                                                                           \\ \cline{2-5} 
                                                                                           & ResNet20                      & PGD                                                & 0.556                                                       & 1.00                                                                           \\ \cline{2-5} 
                                                                                           & \multicolumn{4}{c|}{\textbf{Adaptive Attacks}}                                                                                                                                                                                    \\ \cline{2-5} 
                                                                                           & \multicolumn{1}{l|}{ResNet20} & n=3                                                & 0.505                                                       & 0.80                                                                           \\ \cline{2-5} 
                                                                                           & ResNet20                      & Noise $\lambda=0.05$                               & 0.510                                                       & 0.79                                                                           \\ \cline{2-5} 
                                                                                           & ResNet20                      & Noise $\lambda=0.10$                               & 0.498                                                       & 0.73                                                                           \\ \cline{2-5} 
                                                                                           & ResNet20                      & Noise $\lambda=0.20$                               & 0.467                                                       & 0.64                                                                           \\ \cline{2-5} 
                                                                                           & ResNet20                      & Noise $\lambda=0.30$                               & 0.365                                                       & 0.50                                                                           \\ \cline{2-5} 
                                                                                           & ResNet20                      & Noise $\lambda=0.40$                               & 0.190                                                       & 0.21                                                                           \\ \cline{2-5} 
                                                                                           & ResNet20                      & Noise $\lambda=0.50$                               & 0.122                                                       & 0.07                                                                           \\ \cline{2-5} 
                                                                                           & ResNet20                      & Labels $\rho=0.05$                                 & 0.543                                                       & 0.97                                                                           \\ \cline{2-5} 
                                                                                           & ResNet20                      & Labels $\rho=0.10$                                 & 0.528                                                       & 0.89                                                                           \\ \cline{2-5} 
                                                                                           & ResNet20                      & Labels $\rho=0.15$                                 & 0.533                                                       & 0.91                                                                           \\ \cline{2-5} 
                                                                                           & ResNet20                      & Labels $\rho=0.20$                                 & 0.545                                                       & 0.93                                                                           \\ \cline{2-5} 
                                                                                           & ResNet20                      & Labels $\rho=0.25$                                 & 0.539                                                       & 0.88                                                                           \\ \cline{2-5} 
                                                                                           & ResNet20                      & Labels $\rho=0.30$                                 & 0.547                                                       & 0.90                                                                           \\ \cline{2-5} 
                                                                                           & ResNet20                      & Labels $\rho=0.35$                                 & 0.551                                                       & 0.85                                                                           \\ \cline{2-5} 
                                                                                           & ResNet20                      & Labels $\rho=0.40$                                 & 0.543                                                       & 0.83                                                                           \\ \hline
\end{tabular}
